SPEED: Speculative Pipelined Execution for Efficient Decoding

Generative Large Language Models (LLMs) based on the Transformer architecture have recently emerged as a dominant foundation model for a wide range of Natural Language Processing tasks. Nevertheless, their application in real-time scenarios has been highly restricted due to the significant inference latency associated with these models. This is particularly pronounced due to the autoregressive nature of generative LLM inference, where tokens are generated sequentially since each token depends on all previous output tokens. It is therefore challenging to achieve any token-level parallelism, making inference extremely memory-bound. In this work, we propose SPEED, which improves inference efficiency by speculatively executing multiple future tokens in parallel with the current token using predicted values based on early-layer hidden states. For Transformer decoders that employ parameter sharing, the memory operations for the tokens executing in parallel can be amortized, which allows us to accelerate generative LLM inference. We demonstrate the efficiency of our method in terms of latency reduction relative to model accuracy and demonstrate how speculation allows for training deeper decoders with parameter sharing with minimal runtime overhead.

==> _s_4_related_work.tex <==
\section{Related Work}
\label{sec:related-work}

Prior works have explored parameter sharing in encoder-only \cite{lan2020albert}, encoder-decoder \cite{dehghani2019universal}, and decoder-only \cite{reid2021subformer} Transformers as a method for reducing the size of the network by sharing parameters across all layers in the encoder and/or all layers in the decoder. 
\cite{takase2022lessons} explored only sharing parameters amongst a subset of layers and found that cyclic parameter sharing schemes outperformed sharing across all layers.
There have also been several works on speculative decoding which aim to produce a set of ``draft'' tokens autoregressively using a smaller network and then correct them (in parallel) using a larger network  \cite{chen2023accelerating,leviathan2022fast,kim2023big}. 
Our work instead aims to support speculative execution within a single network in order to accelerate inference with parameter sharing networks.

There are also prior works that aim to accelerate decoder inference through early exiting, where inference is terminated early when the model is confident that it can already predict the next token \cite{schuster2022confident, tang2023need}. 
Our work also leverages similar intuition, namely that while certain predictions truly benefit from the models’ full capacity, other continuations are more trivial and can be solved with reduced compute \cite{schuster2022confident}.
However, our proposed approach for accelerating decoder inference has advantages over typical early exiting approaches. 
Although early exit can be applied to an existing network and doesn't require pretraining, our method is guaranteed to always achieve the same accuracy as the baseline network with parameter sharing since it fixes any mistakes. 
Our method also reduces the model size through parameter sharing (in addition to the speedup from pipelined execution).
